Trikarenos: A Fault-Tolerant RISC-V-based Microcontroller for CubeSats in 28nm

One of the key challenges when operating microcontrollers in harsh environments such as space is radiation-induced Single Event Upsets (SEUs), which can lead to errors in computation. Common countermeasures rely on proprietary radiation-hardened technologies, low density technologies, or extensive replication, leading to high costs and low performance and efficiency. To combat this, we present Trikarenos, a fault-tolerant 32-bit RISC-V microcontroller SoC in an advanced TSMC 28nm technology. Trikarenos alleviates the replication cost by employing a configurable triple-core lockstep configuration, allowing three Ibex cores to execute applications reliably, operating on ECC-protected memory. If reliability is not needed for a given application, the cores can operate independently in parallel for higher performance and efficiency. Trikarenos consumes 15.7mW at 250MHz executing a fault-tolerant matrix-matrix multiplication, a 21.5x efficiency gain over state-of-the-art, and performance is increased by 2.96x when reliability is not needed for processing, with a 2.36x increase in energy efficiency.

==> fig/plot_power_nominal_voltage.tex <==


    \pgfplotstableread{
    Frequency Idle Locked Single Parallel
    0         2.38   2.38   2.38     2.38
    100       4.32   7.65   5.48     9.32
    150       5.3   10.35   7.08    12.80
    200       6.29  13.02   8.69    16.24
    250       7.27  15.68  10.29    19.69
    275       7.77  17.01  11.09    21.06
    }\newpowerdata
    \begin{tikzpicture}
        \begin{axis}[
            width=\columnwidth,
            height=6cm,
            xmin=0,
            xmax=300,
            xlabel={Frequency [\si{\mega\hertz}]},
            ylabel={Core Power [\si{\milli\watt}]},
            legend style={at={(axis cs:8, 22.5)},anchor=north west},
            y label style={at={(axis description cs:0.1,.5)},rotate=0,anchor=south}
        ]
            \addplot[
                color=PULPgreen,
                mark=square,
                only marks,
                very thick
            ] table [x=Frequency, y=Parallel] {\newpowerdata};
            \addlegendentry{Parallel Cores}
            \addplot[color=PULPgreen, domain=0:275, forget plot] ({x},{0.0693*x+2.38});
            \addplot[
                color=PULPred,
                mark=square,
                only marks,
                very thick
            ] table [x=Frequency, y=Locked] {\newpowerdata};
            \addlegendentry{Locked Cores}
            \addplot[color=PULPred, domain=0:275, forget plot] ({x},{0.053*x+2.38});
            \addplot[
                color=PULPorange,
                mark=square,
                only marks,
                very thick
            ] table [x=Frequency, y=Single] {\newpowerdata};
            \addlegendentry{Single Core}
            \addplot[color=PULPorange, domain=0:275, forget plot] ({x},{0.0316*x+2.38});
            \addplot[
                color=PULPblue,
                mark=square,
                only marks,
                very thick
                ]
                table [x=Frequency, y=Idle] {\newpowerdata};
            \addlegendentry{Idle}
            \addplot[color=PULPblue, domain=0:275, forget plot] ({x},{0.0196*x+2.38});
            \addplot[color=PULPpurple, domain=0:300] ({x},{2.38});
            \addlegendentry{Leakage}
        \end{axis}
    \end{tikzpicture}
    \caption{Power measurement results of a 24x24 32-bit Matrix multiplication for different \gls{odrg} configurations at nominal voltage.}
    \label{fig:matmul_pwr}

